Federated Learning Framework Coping with Hierarchical Heterogeneity in Cooperative ITS

Deep learning is a key approach for the environment perception function of Cooperative Intelligent Transportation Systems (C-ITS) with autonomous vehicles and smart traffic infrastructure. In today's C-ITS, smart traffic participants are capable of timely generating and transmitting a large amount of data. However, these data can not be used for model training directly due to privacy constraints. In this paper, we introduce a federated learning framework coping with Hierarchical Heterogeneity (H2-Fed), which can notably enhance the conventional pre-trained deep learning model. The framework exploits data from connected public traffic agents in vehicular networks without affecting user data privacy. By coordinating existing traffic infrastructure, including roadside units and road traffic clouds, the model parameters are efficiently disseminated by vehicular communications and hierarchically aggregated. Considering the individual heterogeneity of data distribution, computational and communication capabilities across traffic agents and roadside units, we employ a novel method that addresses the heterogeneity of different aggregation layers of the framework architecture, i.e., aggregation in layers of roadside units and cloud. The experiment results indicate that our method can well balance the learning accuracy and stability according to the knowledge of heterogeneity in current communication networks. Comparing to other baseline approaches, the evaluation on federated datasets shows that our framework is more general and capable especially in application scenarios with low communication quality. Even when 90% of the agents are timely disconnected, the pre-trained deep learning model can still be forced to converge stably, and its accuracy can be enhanced from 68% to over 90% after convergence.

==> sections/00_abstract.tex <==
\begin{abstract}
Deep learning powered object detection method is the key of environment perception for autonomous driving and smart traffic in Cooperative Intelligent Transportation Systems (C-ITS). 
However, the performance of the detection is strongly dependent on the data volume in model training, which is usually not sufficient due to the limited data collected by specific testing vehicles. 
Meanwhile, all intelligent traffic participants can generate a large number of data timely, which can not be used directly, because of privacy issue.
In this paper, we introduce a two-tier federated learning framework, which can notable enhance OEM pre-trained deep learning model by exploiting data from connected public traffic agents in vehicular networks without affecting the user data privacy. 
Through coordinating existing traffic infrastructure, including roadside units and traffic cloud, the model parameters are disseminated by V2X communication and aggregated hierarchically.
With consideration of individual heterogeneity of data distribution and computation ability across traffic agents, we employ a novel method that addresses the fairness problem in different layers of framework architecture, i.e. traffic agent- and roadside unit layer.
Finally, We show the model enhancement in real traffic scenarios by running deep learning methods in federated fashion and demonstrate our proposal of federated object detection in with traffic image data. The simulation results show that the perception accuracy is on average improved by around \Crs{xx\%} with \Crs{xx\%} less communication time.
\end{abstract}

%\begin{IEEEkeywords}
%federated learning, deep learning model enhancement, cooperative intelligent transportation system, traffic object detection, image processing
%\end{IEEEkeywords}

==> sections/00_abstract_v2.tex <==
\begin{abstract}

Deep learning is a key approach for object detection in the environment perception function of Cooperative Intelligent Transportation Systems (C-ITS) with autonomous vehicles and a smart traffic infrastructure. %
The performance of the object detection strongly depends on the data volume in the model training, which is usually not sufficient due to the limited data collected by a typically small fleet of test vehicles. %
In today's C-ITS, smart traffic participants are capable to timely generate and transmit a large amount of data. However, these data can not be used for model training directly due to privacy constraints. %
In this paper, we introduce a Hierarchical Heterogeneity-tolerated federated learning (HHt-Fed) framework, which can notably enhance the conventional %OEM 
pre-trained deep learning model. The framework exploits data from connected public traffic agents in vehicular networks without affecting the user data privacy. 
Through coordinating existing traffic infrastructure, including roadside units and traffic clouds, the model parameters are efficiently disseminated by vehicular communications and hierarchically aggregated.
Considering the individual heterogeneity of data distribution, computational capabilities across traffic agents, we employ a novel method that addresses the fairness problem at different layers of the framework architecture, i.e., the traffic agent layer and the roadside unit layer.
Finally, we show the model enhancement in real traffic scenarios by running deep learning methods in a federated fashion and demonstrate our proposal of federated object detection with traffic image data. The simulation results show that the perception accuracy is improved on average by around \Crs{xx\%} after only \Crs{xx} communication rounds.
\end{abstract}

\begin{IEEEkeywords}
federated learning, deep learning model enhancement, cooperative intelligent transportation system, traffic object detection, image processing
\end{IEEEkeywords}

==> sections/00_abstract_v3.tex <==
\begin{abstract}

Deep learning is a key approach for object detection in the environment perception function of Cooperative Intelligent Transportation Systems (C-ITS) with autonomous vehicles and a smart traffic infrastructure. %
The performance of the object detection strongly depends on the data volume in the model training, which is usually not sufficient due to the limited data collected by a typically small fleet of test vehicles. %
In today's C-ITS, smart traffic participants are capable to timely generate and transmit a large amount of data. However, these data can not be used for model training directly due to privacy constraints. %
In this paper, we introduce a federated learning framework coping with Hierarchical Heterogeneity (\emph{H2Fed}), which can notably enhance the conventional %OEM 
pre-trained deep learning model. The framework exploits data from connected public traffic agents in vehicular networks without affecting the user data privacy. 
Through coordinating existing traffic infrastructure, including roadside units and road traffic clouds, the model parameters are efficiently disseminated by vehicular communications and hierarchically aggregated.
Considering the individual heterogeneity of data distribution, computational and communication capabilities across traffic agents and roadside units, we employ a novel method that addresses the fairness problem at different aggregation layers of the framework architecture, i.e., aggregation in layers of roadside units and cloud. %
%Finally, the experiment results 
The simulation results indicate that the model is enhanced up to xx\% by applying federated learning in our framework. Even when 80\,\% of the agents are timely disconnected, the learning stability compared to the baseline methods is still increased by up to xx\,\% and learning speed is raised up to xx\,\%.
%\Crs{Finally, we show the model enhancement in real traffic scenarios by running deep learning methods in a federated fashion and demonstrate our proposal of federated object detection with traffic image data. }
%The simulation results show that the perception accuracy is improved on average by around \Crs{xx\%} after only \Crs{xx} communication rounds.
\end{abstract}

\begin{IEEEkeywords}
federated learning, deep learning model enhancement, cooperative ITS, road environmental perception, image processing
\end{IEEEkeywords}
